Predicting Surgery Duration with Neural Heteroscedastic Regression

Scheduling surgeries is a challenging task due to the fundamental uncertainty of the clinical environment, as well as the risks and costs associated with under- and over-booking. We investigate neural regression algorithms to estimate the parameters of surgery case durations, focusing on the issue of heteroscedasticity. We seek to simultaneously estimate the duration of each surgery, as well as a surgery-specific notion of our uncertainty about its duration. Estimating this uncertainty can lead to more nuanced and effective scheduling strategies, as we are able to schedule surgeries more efficiently while allowing an informed and case-specific margin of error. Using surgery records %from the UC San Diego Health System, from a large United States health system we demonstrate potential improvements on the order of 20% (in terms of minutes overbooked) compared to current scheduling techniques. Moreover, we demonstrate that surgery durations are indeed heteroscedastic. We show that models that estimate case-specific uncertainty better fit the data (log likelihood). Additionally, we show that the heteroscedastic predictions can more optimally trade off between over and under-booking minutes, especially when idle minutes and scheduling collisions confer disparate costs.

==> sections/conclusion.tex <==
We demonstrate the efficacy of heteroscedastic neural regression for predicting surgery duration. Our best models improve upon current practice, reducing MAE by $19.8\%$. This work could potentially lead to greater throughput and lower costs in the operating room. 
% We provide further analysis in Appendix \ref{sec:economic}, demonstrating that each model could be used to trade off between over-reserved and under-reserved minutes. 
The uncertainty information from heteroscedastic models can aid decision theory. As determined by negative log likelihood, our analysis shows that the heteroscedastic Laplace MLP dominates the other models.


